Effective Self-supervised Pre-training on Low-compute Networks without Distillation

Despite the impressive progress of self-supervised learning (SSL), its applicability to low-compute networks has received limited attention. Reported performance has trailed behind standard supervised pre-training by a large margin, barring self-supervised learning from making an impact on models that are deployed on device. Most prior works attribute this poor performance to the capacity bottleneck of the low-compute networks and opt to bypass the problem through the use of knowledge distillation (KD). In this work, we revisit SSL for efficient neural networks, taking a closer at what are the detrimental factors causing the practical limitations, and whether they are intrinsic to the self-supervised low-compute setting. We find that, contrary to accepted knowledge, there is no intrinsic architectural bottleneck, we diagnose that the performance bottleneck is related to the model complexity vs regularization strength trade-off. In particular, we start by empirically observing that the use of local views can have a dramatic impact on the effectiveness of the SSL methods. This hints at view sampling being one of the performance bottlenecks for SSL on low-capacity networks. We hypothesize that the view sampling strategy for large neural networks, which requires matching views in very diverse spatial scales and contexts, is too demanding for low-capacity architectures. We systematize the design of the view sampling mechanism, leading to a new training methodology that consistently improves the performance across different SSL methods (e.g. MoCo-v2, SwAV, DINO), different low-size networks (e.g. MobileNetV2, ResNet18, ResNet34, ViT-Ti), and different tasks (linear probe, object detection, instance segmentation and semi-supervised learning). Our best models establish a new state-of-the-art for SSL methods on low-compute networks despite not using a KD loss term.

==> tables/ablation_arch_small.tex <==
\begin{tabular}{l|ll}
\toprule
\multirow{2.5}{*}{Method} &\multicolumn{2}{c}{Linear eval. on ImageNet-1k}\\ 
\cmidrule{2-3}  %\cline{2-8} 
& Top-1(\%) & Top-5(\%)\\
\toprule 
 & \multicolumn{2}{c}{MobileNetV2 ({\scriptsize $\mathtt{\# Par.}2.2$M; $\mathtt{GFLOPS}~0.31$})}\\
Supervised & 71.9 & 90.3 \\
DINO & 66.2 & 86.4  \\
Ours & 68.3 {\footnotesize (\textcolor{ForestGreen}{+2.1})} & 87.8 {\footnotesize (\textcolor{ForestGreen}{+1.4})}  \\
\midrule
 & \multicolumn{2}{c}{ResNet18 ({\scriptsize $\mathtt{\# Par.}11.2$M; $\mathtt{GFLOPS}~1.8$})}\\
Supervised & 69.8 & 89.1 \\
DINO & 62.2 & 84.0 \\
Ours & 65.7 {\footnotesize (\textcolor{ForestGreen}{+3.5})} & 86.6 {\footnotesize (\textcolor{ForestGreen}{+2.6})}\\
\midrule
 & \multicolumn{2}{c}{ViT-Ti/32 ({\scriptsize $\mathtt{\# Par.}5.5$M; $\mathtt{GFLOPS}~0.31$})}\\
Supervised & - & - \\
DINO & 55.4 & 78.1 \\
Ours & 60.1 {\footnotesize (\textcolor{ForestGreen}{+4.7})} & 81.8 {\footnotesize (\textcolor{ForestGreen}{+3.7})} \\
\bottomrule
\end{tabular}

==> tables/ablation_backbone.tex <==
% \begin{tabular}{l|ll|ll}
% \toprule
% \multirow{2.5}{*}{Backbone} &\multicolumn{2}{c|}{Linear eval. on ImageNet-1k}&\multicolumn{2}{c}{Linear eval. on ImageNet-1k}\\ 
% \cmidrule{2-5}  %\cline{2-8} 
% & Top-1(\%) & Top-5(\%) & Top-1(\%) & Top-5(\%) \\
% % \midrule
% \toprule %\shline
%  & \multicolumn{2}{c|}{\textit{MobileNetV2}} & \multicolumn{2}{c}{\textit{ResNet34}} \\
%  & \multicolumn{2}{c|}{({\scriptsize $\mathtt{\# Par.}2.2$M; $\mathtt{GFLOPS}~0.31$})} & \multicolumn{2}{c}{({\scriptsize $\mathtt{\# Par.}21.3$M; $\mathtt{GFLOPS}~3.67$})}\\
% Supervised & 71.9 & 90.3 & 73.3 & 91.4 \\
% DINO baseline & 66.2 & 86.4 & 67.7 & 88.4\\
% Ours & 68.3 {\footnotesize (\textcolor{ForestGreen}{+2.1})} & 87.8 {\footnotesize (\textcolor{ForestGreen}{+1.4})} & 69.7 {\footnotesize (\textcolor{ForestGreen}{+2.0})} & 89.5 {\footnotesize (\textcolor{ForestGreen}{+1.1})}\\
% \midrule
% & \multicolumn{2}{c|}{\textit{ResNet18}} & \multicolumn{2}{c}{\textit{ResNet50}}\\
% & \multicolumn{2}{c|}{({\scriptsize $\mathtt{\# Par.}11.2$M; $\mathtt{GFLOPS}~1.8$})} & \multicolumn{2}{c}{({\scriptsize $\mathtt{\# Par.}23.5$M; $\mathtt{GFLOPS}~4.12$})}\\
% Supervised & 69.8 & 89.1 & 76.1 & 92.9 \\
% DINO baseline & 62.2 & 84.0 & 73.4 & 91.5\\
% Ours & 65.7 {\footnotesize (\textcolor{ForestGreen}{+3.5})} & 86.6 {\footnotesize (\textcolor{ForestGreen}{+2.6})} & 73.4 {\footnotesize (\textcolor{ForestGreen}{+0.0})} & 91.5 {\footnotesize (\textcolor{ForestGreen}{+0.0})}\\
% \bottomrule
% \end{tabular}


% \begin{tabular}{l|ll|ll}
% \toprule
% \multirow{2.5}{*}{Backbone} &\multicolumn{4}{c}{Linear eval. on ImageNet-1k}\\ 
% \cmidrule{2-5}  %\cline{2-8} 
% & Top-1(\%) & Top-5(\%) & Top-1(\%) & Top-5(\%) \\
% % \midrule
% \toprule %\shline
%  & \multicolumn{2}{c|}{\textit{MobileNetV2}} & \multicolumn{2}{c}{\textit{ResNet34}} \\
%  & \multicolumn{2}{c|}{({\scriptsize $\mathtt{\# Par.}2.2$M; $\mathtt{GFLOPS}~0.31$})} & \multicolumn{2}{c}{({\scriptsize $\mathtt{\# Par.}21.3$M; $\mathtt{GFLOPS}~3.67$})}\\
% Supervised & 71.9 & 90.3 & 73.3 & 91.4 \\
% \textit{DINO} & 66.2 & 86.4 & 67.7 & 88.4\\
% Ours & 68.3 {\footnotesize (\textcolor{ForestGreen}{+2.1})} & 87.8 {\footnotesize (\textcolor{ForestGreen}{+1.4})} & 69.7 {\footnotesize (\textcolor{ForestGreen}{+2.0})} & 89.5 {\footnotesize (\textcolor{ForestGreen}{+1.1})}\\
% \midrule
% & \multicolumn{2}{c|}{\textit{ResNet18}} & \multicolumn{2}{c}{\textit{ResNet50}}\\
% & \multicolumn{2}{c|}{({\scriptsize $\mathtt{\# Par.}11.2$M; $\mathtt{GFLOPS}~1.8$})} & \multicolumn{2}{c}{({\scriptsize $\mathtt{\# Par.}23.5$M; $\mathtt{GFLOPS}~4.12$})}\\
% Supervised & 69.8 & 89.1 & 76.1 & 92.9 \\
% \textit{DINO} & 62.2 & 84.0 & 73.4 & 91.5\\
% Ours & 65.7 {\footnotesize (\textcolor{ForestGreen}{+3.5})} & 86.6 {\footnotesize (\textcolor{ForestGreen}{+2.6})} & 73.4 {\footnotesize (\textcolor{ForestGreen}{+0.0})} & 91.5 {\footnotesize (\textcolor{ForestGreen}{+0.0})}\\
% \midrule
% & \multicolumn{2}{c|}{\textit{ViT-Ti/16}} & \multicolumn{2}{c}{\textit{ViT-S/16}}\\
% & \multicolumn{2}{c|}{({\scriptsize $\mathtt{\# Par.}5.5$M; $\mathtt{GFLOPS}~1.26$})} & \multicolumn{2}{c}{({\scriptsize $\mathtt{\# Par.}21.7$M; $\mathtt{GFLOPS}~4.61$})}\\
% Supervised & 72.2 & 91.1 & 79.9 & 95.0 \\
% \textit{DINO}  & 66.7 & 86.6 & 75.4 & 92.3\\
% Ours & 69.5 {\footnotesize (\textcolor{ForestGreen}{+2.8})} & 88.5 {\footnotesize (\textcolor{ForestGreen}{+1.9})} & 76.1 {\footnotesize (\textcolor{ForestGreen}{+0.7})} & 92.7 {\footnotesize (\textcolor{ForestGreen}{+0.4})}\\
% \bottomrule
% \end{tabular}


\begin{tabular}{l|ll|ll|ll}
\toprule
\multirow{2.5}{*}{Backbone} &\multicolumn{6}{c}{Linear eval. on ImageNet-1k}\\ 
\cmidrule{2-7}  %\cline{2-8} 
& Top-1(\%) & Top-5(\%) & Top-1(\%) & Top-5(\%) & Top-1(\%) & Top-5(\%)\\
\toprule %\shline
 & \multicolumn{2}{c|}{MobileNetV2} & \multicolumn{2}{c|}{ResNet18} & \multicolumn{2}{c}{ViT-Ti/16} \\
 & \multicolumn{2}{c|}{({\scriptsize $\mathtt{\# Par.}2.2$M; $\mathtt{GFLOPS}~0.31$})} & \multicolumn{2}{c|}{({\scriptsize $\mathtt{\# Par.}11.2$M; $\mathtt{GFLOPS}~1.8$})} & \multicolumn{2}{c}{({\scriptsize $\mathtt{\# Par.}5.5$M; $\mathtt{GFLOPS}~1.26$})}\\
Supervised & 71.9 & 90.3 & 69.8 & 89.1 & 72.2 & 91.1 \\
DINO & 66.2 & 86.4 & 62.2 & 84.0 & 66.7 & 86.6 \\
Ours & 68.3 {\footnotesize (\textcolor{ForestGreen}{+2.1})} & 87.8 {\footnotesize (\textcolor{ForestGreen}{+1.4})} & 65.7 {\footnotesize (\textcolor{ForestGreen}{+3.5})} & 86.6 {\footnotesize (\textcolor{ForestGreen}{+2.6})} & 69.5 {\footnotesize (\textcolor{ForestGreen}{+2.8})} & 88.5 {\footnotesize (\textcolor{ForestGreen}{+1.9})} \\
\toprule %\shline
 & \multicolumn{2}{c|}{ResNet34} & \multicolumn{2}{c|}{ResNet50} & \multicolumn{2}{c}{ViT-S/16} \\
 & \multicolumn{2}{c|}{({\scriptsize $\mathtt{\# Par.}21.3$M; $\mathtt{GFLOPS}~3.67$})} & \multicolumn{2}{c|}{({\scriptsize $\mathtt{\# Par.}23.5$M; $\mathtt{GFLOPS}~4.12$})} & \multicolumn{2}{c}{({\scriptsize $\mathtt{\# Par.}21.7$M; $\mathtt{GFLOPS}~4.61$})}\\
Supervised & 73.3 & 91.4 & 76.1 & 92.9 & 79.9 & 95.0  \\
DINO & 67.7 & 88.4 & 73.4 & 91.5 & 75.4 & 92.3 \\
Ours & 69.7 {\footnotesize (\textcolor{ForestGreen}{+2.0})} & 89.5 {\footnotesize (\textcolor{ForestGreen}{+1.1})}& 73.4 {\footnotesize (\textcolor{ForestGreen}{+0.0})} & 91.5 {\footnotesize (\textcolor{ForestGreen}{+0.0})} & 76.1 {\footnotesize (\textcolor{ForestGreen}{+0.7})} & 92.7 {\footnotesize (\textcolor{ForestGreen}{+0.4})} \\
\bottomrule
\end{tabular}

==> tables/ablation_nviews.tex <==
\begin{tabular}{lllll}
\toprule
$\mathtt{LC}$ & $\mathtt{S}$ & \# Views  & $\overline{\mathtt{aIoU}}$ & Accu.\\ 
\toprule %\shline
96 & 0.14 & 6 & 0.48 & 65.9 \\
96 & 0.14 & 9 & - & 65.9 \\
96 & 0.14 & 12 & - & 66.2 \\
96 & 0.14 & 20 & 0.50 & 66.3 \\
\midrule
103 & 0.14 & 6 & - & 66.3 \\
103 & 0.14 & 9 & - & 66.8 \\
103 & 0.14 & 12 & - & 66.9 \\
103 & 0.14 & 20 & - & 66.9 \\
\midrule
128 & 0.3 & 3 & - & 67.0 \\
128 & 0.3 & 6 & - & 67.8 \\
128 & 0.3 & 8 & - & 67.9 \\
\bottomrule
\end{tabular}

==> tables/sota_im1k_small.tex <==
\begin{tabular}{l|l|l|l}
\toprule
{Method} & {MobileNetV2} &{ResNet18} &{ResNet34} \\ 
& Top-1 & Top-1 & Top-1 \\
\toprule 
Supervised 71.9 & 69.8 & 73.3 \\
\midrule
\cite{effssl_aaai22} & - & 55.7 & - \\
ReSSL & - 58.1 & - \\
\midrule
CompRess & 65.8  & 62.6 & - \\
SimReg   & \textbf{69.1} & 65.1 & - \\
\midrule
SEED     & - & 59.5 &62.7 \\
DisCo    & - & 65.5 &68.1 \\
BINGO    & - & \underline{65.9} &\underline{69.1} \\
\midrule 
{Ours} & \underline{68.8} {\footnotesize (\textcolor{darkred}{-0.3})} & \textbf{66.8} {\footnotesize (\textcolor{ForestGreen}{+0.9})} & \textbf{70.8} {\footnotesize (\textcolor{ForestGreen}{+1.7})}\\
\bottomrule
\end{tabular}
